Multi-View 3D Object Detection Network for Autonomous Driving

This paper aims at high-accuracy 3D object detection in autonomous driving scenario. We propose Multi-View 3D networks (MV3D), a sensory-fusion framework that takes both LIDAR point cloud and RGB images as input and predicts oriented 3D bounding boxes. We encode the sparse 3D point cloud with a compact multi-view representation. The network is composed of two subnetworks: one for 3D object proposal generation and another for multi-view feature fusion. The proposal network generates 3D candidate boxes efficiently from the bird's eye view representation of 3D point cloud. We design a deep fusion scheme to combine region-wise features from multiple views and enable interactions between intermediate layers of different paths. Experiments on the challenging KITTI benchmark show that our approach outperforms the state-of-the-art by around 25% and 30% AP on the tasks of 3D localization and 3D detection. In addition, for 2D detection, our approach obtains 10.3% higher AP than the state-of-the-art on the hard data among the LIDAR-based methods.

==> table.tex <==
\iffalse
\begin{table*}[t!]
\vspace{-1mm}
\begin{center}
\begin{small}
\addtolength{\tabcolsep}{-0pt}
\begin{tabular}{|c|c||c|c|c|}
\hline
Method & Data & Easy & Moderate & Hard \\
\hline
Mono3D~\cite{XiaozhiCVPR16} & Mono & 93.89 & 88.67 & 79.68 \\
3DOP~\cite{XiaozhiNIPS15} & Stereo & 93.08 & 88.07 & 79.39 \\
%\hline
%Vote3Deep~\cite{vote3deep} & LIDAR & 76.79 & 68.24 & 63.23 \\
\hline
%MV3D (Ours) & BV & 76.40 & 69.92 & 57.47 \\
%MV3D (Ours) & BV+RGB & 76.40 & 69.92 & 57.47 \\
MV3D (Ours) & BV+RGB+FV & {\bf 95.01} & 87.59 & 79.90 \\
\hline
\end{tabular}
\end{small}
\vspace{-2.5mm}
\caption{Average Precision (AP$_{\text{2D}}$) (in \%) on the {\it validation} set of the KITTI Object Detection Benchmark.}
\label{tab:ap_test}
\end{center}
\vspace{-5mm}
\end{table*}
\fi






\iffalse
\begin{table*}[t!]
\begin{center}
%\vspace{-0.3cm}
%\hspace{-0.3cm}
\begin{small}
\addtolength{\tabcolsep}{-0pt}
\begin{tabular}{|c||c|c|c||c|c|c||c|c|c|}
\hline
& \multicolumn{3}{|c||}{Cars} & \multicolumn{3}{|c||}{Pedestrians} & \multicolumn{3}{|c|}{Cyclists} \\
\hline
& Easy & Moderate & Hard & Easy & Moderate & Hard & Easy & Moderate & Hard \\
\hline
% CNN  & 22.19  & 	 15.96  & 13.12  & 11.44  &  9.52  & 8.93   & 19.75  &  19.99  & 18.11   \\
% CSoR  & 33.97  & 25.38  & 21.95  &  - &  - &  -   & - &  - &  - \\
%SVM-Res & 35.02  & 30.38  & 24.87  &   &   &     &   &   &   \\
%VC & 35.45  & 34.00  & 31.89  &  & - & - & - & - & - & -  \\
%DeepInsight & 33.82  & 36.92  & 32.60   & - & - & - & - & - & -  \\
%AOG~\cite{CarAOG_ECCV2014} & 43.81  & 38.21  & 31.53  & - & -   &  - &  - &  - & - \\
AOG~\cite{CarAOG_ECCV2014} & 33.79 & 30.77 & 24.75  & - & -   &  - &  - &  - & - \\
%DPM-C8B1~\cite{ref:Yebes14iv} & 59.51  & 50.32  & 39.22   & 31.08  &  23.37  & 20.72  & 27.25  &  19.25  & 17.95  \\
%ANM & - & - & - & 37.18  & 30.34  & 28.34  &  -  &  -    &   -  \\
LSVM-MDPM-sv~\cite{Geiger11,dpm} & 67.27  & 55.77  & 43.59   & 43.58  & 35.49  & 32.42  &  27.54  & 22.07  & 21.45  \\
DPM-VOC+VP~\cite{PepikPAMI15} & 72.28  & 61.84  & 46.54   & 53.55 & 39.83  & 35.73 & 30.52  &  23.17  & 21.58  \\
OC-DPM~\cite{bojan13cvpr} &  73.50  &  64.42  & 52.40  &  - &  - &  -   &  - &  - &  - \\
%SS  &  83.87  & 73.06  & 58.38  &   &     &   &   &   &  \\
SubCat~\cite{BarTITS15} & 83.41  & 74.42  & 58.83   & 44.32  &  34.18  & 30.76  & -  &  -  &  -   \\
3DVP~\cite{xiangcvpr15} & 86.92 &  74.59  & 64.11   & - & - & - & - & - & - \\
\hline
Ours & {\bf 91.01} & {\bf 86.62} & {\bf 76.84} &{\bf 71.15} & {\bf 58.15} & {\bf 54.94} & {\bf 65.56} & {\bf 54.97} & {\bf 48.77} \\
\hline
\end{tabular}
\end{small}
\vspace{-2mm}
\caption{AOS scores (in \%) on the test set of KITTI's Object Detection and Orientation Estimation Benchmark.}
\label{tab:aos_test}
\vspace{-4mm}
\end{center}
\end{table*}
\fi

